RUBi: Reducing Unimodal Biases in Visual Question Answering

Visual Question Answering (VQA) is the task of answering questions about an image. Some VQA models often exploit unimodal biases to provide the correct answer without using the image information. As a result, they suffer from a huge drop in performance when evaluated on data outside their training set distribution. This critical issue makes them unsuitable for real-world settings. We propose RUBi, a new learning strategy to reduce biases in any VQA model. It reduces the importance of the most biased examples, i.e. examples that can be correctly classified without looking at the image. It implicitly forces the VQA model to use the two input modalities instead of relying on statistical regularities between the question and the answer. We leverage a question-only model that captures the language biases by identifying when these unwanted regularities are used. It prevents the base VQA model from learning them by influencing its predictions. This leads to dynamically adjusting the loss in order to compensate for biases. We validate our contributions by surpassing the current state-of-the-art results on VQA-CP v2. This dataset is specifically designed to assess the robustness of VQA models when exposed to different question biases at test time than what was seen during training. Our code is available: github.com/cdancette/rubi.bootstrap.pytorch

==> sections/_del.tex <==

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{l ccccc}
    \toprule
    Model & RUBi & Rank-Corr. & Overall \\
    
    \midrule
    Random \cite{vqahat} & & 0.000 & \\
    Human \cite{vqahat} & & 0.623 & \\
    \midrule
    % \multirow{2}{*}{Baseline} 
    %     & \xmark & 0.4321           & \\
    %     & \cmark & \textbf{0.4433}  & \\
    % \midrule
    
     \multirow{2}{*}{Baseline}
        % logs/vqa1/murel_small_mlp_no_residual/vqa_hat_spearmanr_sum_epoch0.txt (best)
        & \xmark & 0.431 & 62.89 \\
        % logs/vqa1/murel_small_late_fusion_multiloss_best/vqa_hat_spearmanr_sum_epoch0.txt
        & \cmark & \textbf{0.443}  & 59.27 \\
    \midrule
    
    % \multirow{2}{*}{SAN} 
    %     % logs/vqa1/san/san_vgg16_baseline
    %     & \xmark &  0.2098          &  \\
    %     & \cmark & \textbf{0.2123}  &  \\
    % \midrule
    
    \multirow{2}{*}{SAN}
        % logs/vqa1/san/san_vgg16_baseline/vqa_hat_spearmanr_epoch_0.txt  (best)
        & \xmark & 0.191 & 54.25 \\
        % logs/vqa1/san/san_reproduction_loss_mm_q,loss_q_big_q/vqa_hat_spearmanr_epoch_0.txt
        & \cmark & \textbf{0.210} & 51.28 \\
    \midrule
    
    \multirow{2}{*}{UpDn} 
        % logs/vqa1/updown_corrected/updown_baseline
        &  \xmark & \textbf{0.449} & 61.41  \\
        % logs/vqa1/updown_corrected/updown_glove_loss_mm_q,q_optim_lr,0.001,1.0,1.0,5.0_seed_567
        & \cmark  & 0.446 & 57.72 \\
        
    \bottomrule
    \end{tabular}
    \vspace{0.1cm}
    \caption{Correlation with Human Attention Maps on VQA-HAT \texttt{val} set \cite{vqahat} and overall accuracy top1 on VQA v1 \texttt{val} set.}
    \label{tab:vqahat}
\end{table}{}
\fi

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{l ccccc}
    \toprule
    Model & RUBi & Rank-Corr. & Overall Accuracy \\
    
    \midrule
    Random & & 0.000 & \\
    \midrule
    % \multirow{2}{*}{Baseline} 
    %     & \xmark & 0.4321           & \\
    %     & \cmark & \textbf{0.4433}  & \\
    % \midrule
    
     \multirow{2}{*}{Baseline}
        % logs/vqa1/murel_small_mlp_no_residual/vqa_hat_spearmanr_sum_epoch0.txt (best)
        & \xmark & 0.4307 & 62.89 \\
        % logs/vqa1/murel_small_late_fusion_multiloss_best/vqa_hat_spearmanr_sum_epoch0.txt
        & \cmark & \textbf{0.4424}  & 59.27 \\
    \midrule
    
    % \multirow{2}{*}{SAN} 
    %     % logs/vqa1/san/san_vgg16_baseline
    %     & \xmark &  0.2098          &  \\
    %     & \cmark & \textbf{0.2123}  &  \\
    % \midrule
    
    \multirow{2}{*}{SAN}
        % logs/vqa1/san/san_vgg16_baseline/vqa_hat_spearmanr_epoch_0.txt  (best)
        & \xmark & 0.1909 & 54.25 \\
        % logs/vqa1/san/san_reproduction_loss_mm_q,loss_q_big_q/vqa_hat_spearmanr_epoch_0.txt
        & \cmark & \textbf{0.2098} & 51.28 \\
    \midrule
    
    \multirow{2}{*}{UpDn} 
        % logs/vqa1/updown_corrected/updown_baseline
        &  \xmark & \textbf{0.4496} & 61.41  \\
        % logs/vqa1/updown_corrected/updown_glove_loss_mm_q,q_optim_lr,0.001,1.0,1.0,5.0_seed_567
        & \cmark  & 0.4467 & 57.72 \\
        
    \midrule
    Human & & 0.623 & \\
        
    \bottomrule
    \end{tabular}
    \vspace{0.1cm}
    \caption{Correlation with Human Attention Maps \cite{vqahat} and accuracy on VQA v1 \texttt{val} set.}
    \label{tab:vqahat}
\end{table}{}
\fi 

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{l cc}
    \toprule
    Model & \cmark $\Lqo$ & \xmark $\Lqo$ \\
    \midrule
    Baseline + RUBi & \textbf{47.11} & 46.22 \\
    \midrule
    SAN  + RUBi & \textbf{37.48} & 37.26 \\
    \midrule
    UpDn + RUBi & \textbf{44.23} & 39.47 \\
    \bottomrule \vspace{1mm}
    \end{tabular}
    \caption{Overall accuracy top1 on VQA-CP v2.}
    \label{tab:ablation-lqo}
\end{table}{}
\begin{table}[h]
    \centering
    \begin{tabular}{l cc}
    \toprule
    Model & $\Lmq + \Lqo$ & $\Lmq$ \\
    \midrule
    Baseline + RUBi & \textbf{47.11} & 46.22 \\
    %\midrule
    SAN  + RUBi & \textbf{37.48} & 37.26 \\
    %\midrule
    UpDn + RUBi & \textbf{44.23} & 39.47 \\
    \bottomrule
    \end{tabular}
    \vspace{0.1cm}
    \caption{Overall accuracy top1 on VQA-CP v2, with or without using $\Lqo$ in the loss function.}
    \label{tab:ablation-lqo}
\end{table}{}
\fi

\vspace{-0.6cm}
 

% A caveat is that the released dataset is not controlled for center bias \cite{vqahat}, more experiments would be needed to confirm the gain on an unbiased dataset.
%The better grounding ability is an interesting side effect of RUBi, which is primarily meant to reduce question biases during training. Nevertheless, Interestingly RUBi slightly improves the grounding ability  While RUBi slightly improves the grounding ability, the gains cannot be solely explained by this factor.  .on all three architectures when they are trained with RUBi. on the rank-correlation with human attention maps.   We report a small improvement of +0.0112 compared with our baseline architecture trained without RUBi. The latter is composed of human attention maps from a subset of the VQA v1 dataset. which is the metric accounting for grounding ability. \red{0.4321} in rank-correlation (higher is better) with our baseline architecture and \red{0.4433} when trained with RUBi. We use the VQA-HAT \cite{vqahat} dataset for this purpose. It is composed of human attention maps from a subset of the VQA v1 dataset. The goal is to find whether the scores improvement on VQA-CP came from a better grounding ability of question words, and see whether our method leads to more interpretable models. The models are trained on VQA v1 train split, and we compare our attention maps on the validation split, following the protocol from \cite{vqahat}. We report \red{0.4321} in rank-correlation (higher is better) with our baseline architecture and \red{0.4433} when trained with RUBi.  Other results are shown in Table \ref{tab:vqahat}. We show consistent but small gains on the correlation with human attention maps.   Also, they show that while we improve slightly grounding, the gains cannot be solely explained by this factor. It is however an interesting side effect, that can lead to better interpretability of VQA models.



\iffalse
\begin{table}[!h]
    \centering
    \begin{tabular}{c cc}
    \toprule
    Model & Without RUBi & With RUBi\\
    \midrule
    SAN             &         0.2098    & \textbf{0.2123} \\
    UpDn            & \textbf{0.4496}   &         0.4362  \\ 
    Baseline (ours) &         0.4321    & \textbf{0.4433} \\
%    \red{Baseline (ours), max} & 0.3325 & \textbf{0.3522} \\
    \bottomrule
    \end{tabular} \vspace{0.1cm} 
    \caption{Correlation with Human Attention Maps \cite{vqahat}}
    \label{tab:vqahat-old}
\end{table}
\fi
